HintNet: Hierarchical Knowledge Transfer Networks for Traffic Accident Forecasting on Heterogeneous Spatio-Temporal Data

Traffic accident forecasting is a significant problem for transportation management and public safety. However, this problem is challenging due to the spatial heterogeneity of the environment and the sparsity of accidents in space and time. The occurrence of traffic accidents is affected by complex dependencies among spatial and temporal features. Recent traffic accident prediction methods have attempted to use deep learning models to improve accuracy. However, most of these methods either focus on small-scale and homogeneous areas such as populous cities or simply use sliding-window-based ensemble methods, which are inadequate to handle heterogeneity in large regions. To address these limitations, this paper proposes a novel Hierarchical Knowledge Transfer Network (HintNet) model to better capture irregular heterogeneity patterns. HintNet performs a multi-level spatial partitioning to separate sub-regions with different risks and learns a deep network model for each level using spatio-temporal and graph convolutions. Through knowledge transfer across levels, HintNet archives both higher accuracy and higher training efficiency. Extensive experiments on a real-world accident dataset from the state of Iowa demonstrate that HintNet outperforms the state-of-the-art methods on spatially heterogeneous and large-scale areas.

==> trash.tex <==
\section{MIGHT NOT USED!}
Below is the part might not be used in this paper
====================================================================






\subsection{ Graph Convolutional Layer }
According to the First Law of Geography \cite{GEORGELIU}, there exists stronger traffic spatial auto-correlation between locations and nearby road systems. Inspired by Zhang's work \cite{GEORGELIU}, we apply dynamic convolutional layers on spatial-view and spatial-temporal-view to maximally captures the spatial auto-correlations of traffic accidents along with the road structure.
The layer-wise propagation rule of DyConv is given in Eq. 6.1. The output of each layer is a filtered feature matrix.  


\begin{equation}
H^{R}_{i} = f(H^{R}_{i-1}, A^{R}) = \sigma(A^{R}H^{R}_{i-1}W_{i}), 
\end{equation}

Where $H^{R}_{i}$ is the output feature matrix of region R in i-th layer. $\sigma$ is an activation function and $w_{i}$ is a weight matrix. $A^{R}$ is a row-normalized accident correlation matrix. The accident correlation is used to capture the spatial dependencies between pairs of grids. We use Pearson correlation coefficient\cite{GEORGELIU} by Eq. 6.2 to quantify the accident correlations between grids.

\begin{equation}
a_{XY} = \frac{\sum_{i=1}^n (X_{i}-\overline{X})(Y_{i}-\overline{Y})}{\sqrt{\sum_{i=1}^n (X_{i}-\overline{X})^2 \sum_{i=1}^n (Y_{i}-\overline{Y})^2}}
\end{equation}

where a $\in [-1, 1]$ is the accident correlation for each pair of grids. For an $S \times S$ region, its corresponding correlation matrix, $A^R$, is a symmetric $S^{2} \times S^{2}$ matrix.


In figure 3, the filter in standard Conv has a squared shape and size, and thus covers many cells with low correlation. In opposite, The filter in DyConv generated from accident correlation matrix $A^R$ has an irregular shape, so it exactly covers the structure of road with strong correlation. 

\begin{figure}
    \centering
    \subfloat[Standard Conv Filter]{\includegraphics[width=0.2\textwidth]{standard_con.png}}

	\subfloat[DyCon Filter]{\includegraphics[width=0.2\textwidth]{dycon.PNG}}

	\caption{Filter Comparison between standard Conv and DyConv in the area of Des Moines. Darker color indicates stronger correlation. (pic errors!)}
	\label{spt}
\end{figure}

\subsection{ Local Graph Convolution}
The ideal situation of using DyConv is to generate correlation matrix based on a whole study area. However, it becomes infeasible in a state-wide large-scale grids data, because the training process could be costly in terms of memory for large-scale graphs\cite{GEORGELIU}. Therefore, we borrow the idea from Yao's local CNN method \cite{GEORGELIU} to reduce the the computational cost and improve the training efficiency of our model. 

As shown in Figure ?, in each time interval $t$, we treat each location $i$ and its surrounding neighbor cells as one $S \times S$ image, where the size $S$ controls the spatial granularity and size of correlation matrix $A^R$. $A^R$ is a symmetric $S^{2} \times S^{2}$ matrix. Zero Padding is used on locations at the boundaries of study area. Thus, we for each location $i$ and time interval $t$,  a feature image tensor $X^i_{t}\in \mathbb{R}^{S \times S \times d}$ were retrieved, where $d$ is the dimension of the features. For each feature tensor, there is a corresponding $Y^i_{t}$, where $Y^i_{t}$ is number of accidents in location $i$ and time interval $t$.  
 
 \begin{algorithm2e}
	\SetKwInput{Input}{Input}
	\SetKwInput{Output}{Output}
	\LinesNumbered
	\DontPrintSemicolon
	\BlankLine
	\caption{Risk(density?)-Based Grids Partitioning}
	\label{pseudo_learn}
	\Input{accidents matrix $A$, epsilon $\epsilon$, minimum number of points $\beta$, minimum number of neighbours $\sigma$}
	\Output{cluster label matrix}
	\BlankLine

    RGP($\epsilon$, $\beta$, $\sigma$, $A$):
    $create a unclassified cluster_matrix with same shape as A$
    $cluster\_label = 1$\\
	\For{each grid in cluster\_matrix}
	{
        \If{grid == Unclassified}{
            \If{ExpandCluster(Grid)}{
                cluster\_label ++
            }
        }
    }

    ExpandCluster(grid):\\
    $global cluster\_label$
    $seeds = NeighbourQuery(grid)$\\
    \If{$NeibourCounter(seeds) < min_neighbours$}{
        $cluster\_matrix[grid] = cluster\_label$
        return False
    }
    \Else{
        $cluster\_Matrix[grid] = cluster\_label$\\
        \For{each seed in seeds}{
            $cluster_matrix[seed] = cluster\_label $
        }
    
        \While{seeds is not empty}{
            $current = seeds[0]$\\
            $current\_neighbours = NeighbourQuery(current)$\\
            \If{$NeighbourCounter(current_neighbours, current) >= min_neighbours$}{
                \For{each nei in current\_neighbours}{
                    \If{cluster\_matrix[nei] is Unclassified or cluster\_matrix[nei] is NOISE}{
                        \If{cluster\_matrix[nei] is Unclassified}{
                            $seeds.append(nei)$
                            $cluster\_matrix[seed] = NOISE$
                        }
                        
                    }
                }
            }
            $seeds.pop()$
        }
    return True
    
    NeighbourCounter(current\_neighbours, current):
    $ctr=0$
    \For{each neighbour in current\_neighbours}{
        \If{$accident\_matrix[neighbour] > min_points$}{ $ctr++$ }
    }
    \If{$accident\_matrix[current] > min_points$}{
        $ctr ++$
    }
    return ctr
    
    }
        
\end{algorithm2e}

\begin{table}[]
	\centering
	%\small
	\caption{Number of parameters comparison (in thousand)}
	\begin{tabular}{|c|c|c|c|c|}
		\hline
    		& \textbf{ConvLSTM} & \textbf{GSNet} & \textbf{Ours} &\textbf{Ours}\\
		\hline
		\hline
		$16 \times 16$ &$1,112,211$ & $1,106,454$ &$1,112,211$ & $1,182,580$\\
		\hline
		$32 \times 32$ &$3,088,051$ & $16,835,862$ &$3,088,051$ &$1,182,580$\\
		\hline
		$64 \times 64$ &$6,052,771$ & $268,497,174$ & $27,792,459$ &$2,277,220$\\
		\hline
		$128 \times 64$ &$10,007,523$ & $536,994,348$ & $64,849,071$ & $2,277,220$\\
		\hline
		

	\end{tabular}
	\label{real_data}
\end{table}


\begin{table}[]
	\centering
	%\small
	\caption{Performance comparison on each level}
	\begin{tabular}{|c|c|c|c|}
		\hline
    		& \textbf{HA} & \textbf{Ours} & \textbf{number of cells} \\
		\hline
		\hline
		Level 6 & $0.829$ & $\textbf{0.625}$ & $165$\\
		\hline
		Level 5 &$0.155$ & $\textbf{0.118}$ & $134$\\
		\hline
		Level 4 &$0.082$ & $\textbf{0.066}$ & $185$\\
		\hline
		Level 3 &$0.062$ & $0.049$ & $325$\\
		\hline
		Level 2 &$0.043$ & $0.034$ & $362$\\
		\hline
		Level 1 &$0.008$ & $0.007$ & $1447$\\
		\hline
		Level 0 &$0.000$ & $0.000$ & $5574$\\
		\hline
		ALL &$0.027$ & $\textbf{0.021}$ & $128 \times 64$\\
		\hline
		

	\end{tabular}
	\label{real_data}
\end{table}


are used to reduce time and memory costs. Lastly, the final prediction is based on the concatenation of results from graph convolution layers and LSTM layers. In this way, we can maximally capture inherent relationships between traffic accidents and features temporally and spatially, meanwhile, the computational expense is reduced significantly. 
 
 \textbf{sub-region graph Convolution}
Convolutional Neural Network (ConvNet/CNN) is widely adopted for studying the spatial dependencies on geo-spatial problems as the first law of geography \cite{??}. However, the square-shaped filter in CNN is not appropriate for traffic-related cases as a result of the irregular-shaped road networks. Traffic accidents only occur along with road networks. Therefore, to maximally captures the spatial auto-correlations of traffic accidents along with the road structure, many states of art methods like GSNet \cite{??} takes advantage of Graph Convolution, where cells are treated as vertices and the correlations between cells are treated as edges. However, most related works focus on small areas like Chicago or New York City with a limited size of the graph. It becomes infeasible in a state-wide grid data, because the training process could be costly in terms of memory for large-scale graphs\cite{??}. For example, the grid size of Chicago in GSNet is only $20 \times 20$, but it is $128 \times 64$ in the State of Iowa. The adjacent matrix in this case is $420$ times larger. 

To implement graph convolution on a large-scale map efficiently, we borrow the idea from Yao's local CNN idea \cite{??} and combine it with graph convolution to reduce the computational cost and improve the model accuracy. In each time interval $t$, we treat each location $i$ and its surrounding neighbor cells as one $S \times S$ image, where the size $S$, a hyper parameter, controls the spatial granularity and size of correlation matrix $A^R$. $A^R$ is a symmetric $S^{2} \times S^{2}$ matrix. Zero Padding is used on locations at the boundaries of the study area. Thus, for each location $i$ and time interval $t$,  a feature image tensor $X^i_{t}\in \mathbb{R}^{S \times S \times d}$ were retrieved, where $d$ is the dimension of the features. For each feature tensor, there is a corresponding $Y^i_{t}$, where $Y^i_{t}$ is number of accidents in location $i$ and time interval $t$. The input of the Local graph Convolution layer is sub-regions $X^i_{t}$ for each cell.

\begin{equation}
H^{R}_{i} = f(H^{R}_{i-1}, A^{R}) = \sigma(A^{R}H^{R}_{i-1}W_{i}), 
\end{equation}

Where $H^{R}_{i}$ is the output feature matrix of region R in the i-th layer. $A^{R}$ is a row-normalized accident correlation matrix. Inspired by Zhang's dynamic CNN \cite{??}, We use the Pearson correlation coefficient to quantify the accident correlations between grid cells and capture the spatial dependencies between traffic patterns and the grid. In this way, convolution filters focus more on regions with higher correlations and ignore the regions with dissimilar traffic accident patterns.


\subsection{Long Short-Term Memory(LSTM) (might remove this part)}
LSTM is a type of recurrent neural network that performs well on time-series data with temporal dependencies, so LSTM is used as a building block in our proposed model. LSTM node consists of a memory cell $c_t$, an input gate $i^i_t$, an output gate $o^i_t$, and forget gate $f^i_t$. LSTM takes $g^i_t$, $h_{t-1}$, and $c^i_{t-1}$ as inputs in each time interval $t$. Memory cell is used to pass information from state to state, and forget fate is designed to forget previous memory cell. The LSTM is formulated as follows:

$i^i_t = \sigma(W_{i}g^i_{t} + U_{i}h^i_{t-1}+b_{i}),$\\
$f^i_{t} = \sigma(W_{f}g^i_{t} + U_{f}h^i_{t-1}+b_{f}),$\\
$o^i_{t} = \sigma(W_{o}g^i_{t} + U_{o}h^i_{t-1}+b_{o}),$\\
$\theta^i_{t}=\tanh(W_{o}g^i_{t}+U_{o}h^i_{t-1}+b_{g}),$\\
$c^i_{t} = f^i_{t} \circ c^i_{t-1} + i^i_t \circ  \theta^i_{t}$\\
$h^i_{t} = o^i_{t} \circ \tanh(c^i_{t})$

where the $\circ$ denotes Hadamard product and $W_{a}, U_{a}, b_{a} (a \in {i, f, o, g}) are learnable parameters$. The $h^i_{t}$ is the output of region $i$ of LSTM after $t$ times interval. The Inputs of each hidden state in LSTM layer are the concatenation of outcomes from both temporal feature and spatial-temporal features.

@article{oh2006accident,
  title={Accident prediction model for railway-highway interfaces},
  author={Oh, Jutaek and Washington, Simon P and Nam, Doohee},
  journal={Accident Analysis \& Prevention},
  volume={38},
  number={2},
  pages={346--356},
  year={2006},
  publisher={Elsevier}
}

@article{tamerius2016precipitation,
  title={Precipitation effects on motor vehicle crashes vary by space, time, and environmental conditions},
  author={Tamerius, JD and Zhou, X and Mantilla, R and Greenfield-Huitt, T},
  journal={Weather, Climate, and Society},
  volume={8},
  number={4},
  pages={399--407},
  year={2016},
  publisher={American Meteorological Society}
}

@article{ren2017deep,
  title={A deep learning approach to the prediction of short-term traffic accident risk},
  author={Ren, Honglei and Song, You and Liu, JingXin and Hu, Yucheng and Lei, Jinzhi},
  journal={arXiv preprint arXiv:1710.09543},
  year={2017}
}

\begin{figure}[t]
    \centering
    
    \begin{minipage}{0.2\textwidth}
    \includegraphics[width=1\textwidth]{crash.png}\hfill
    \caption*{(a) traffic accidents in Iowa}
    \end{minipage}\hfill
    \begin{minipage}{0.2\textwidth}
    \includegraphics[width=1\textwidth]{coop.png}
    \caption*{COOP Observation Stations}
    \end{minipage}\hfill
\vspace{-0.1in}
	\caption{Visualization of traffic accidents, road network, and COOP}
	\vspace{-0.1in}
	\label{three_data_map}
\end{figure}
\vspace{-0.1in}


@inproceedings{yuan2018hetero,
  title={Hetero-convlstm: A deep learning approach to traffic accident prediction on heterogeneous spatio-temporal data},
  author={Yuan et al.},
  booktitle={ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={984--992},
  year={2018}
}

@inproceedings{zhou2020riskoracle,
  title={RiskOracle: A Minute-Level Citywide Traffic Accident Forecasting Framework},
  author={Zhou, Zhengyang and Wang, Yang and Xie, Xike and Chen, Lianliang and Liu, Hengchang},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  number={01},
  pages={1258--1265},
  year={2020}
}

@inproceedings{wang2021gsnet,
  title={GSNet: Learning Spatial-Temporal Correlations from Geographical and Semantic Aspects for Traffic Accident Risk Forecasting},
  author={Wang, Beibei and Lin, Youfang and Guo, Shengnan and Wan, Huaiyu},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={5},
  pages={4402--4409},
  year={2021}
}

 @misc{2020fatality, title={2020 fatality data show increased traffic fatalities during pandemic}, url={https://www.nhtsa.gov/press-releases/2020-fatality-data-show-increased-traffic-fatalities-during-pandemic}, journal={NHTSA}, publisher={NHTSA}, author={Media, NHTSA}, year={2021}, month={Jun}}
 
@article{burd2021travel,
  title={Travel time to work in the united states: 2019},
  author={Burd, Charlynn and Burrows, Michael and McKenzie, Brian},
  journal={American Community Survey Reports, United States Census Bureau},
  year={2021}
}

@article{burrows2021commuting,
  title={Commuting by Public Transportation in the United States: 2019},
  author={Burrows, Michael and Burd, Charlynn and McKenzie, Brian},
  journal={American Community Survey Reports, United States Census Bureau},
  year={2021}
}

@article{chang2005analysis,
  title={Analysis of freeway accident frequencies: negative binomial regression versus artificial neural network},
  author={Chang, Li-Yen},
  journal={Safety science},
  volume={43},
  number={8},
  pages={541--557},
  year={2005},
  publisher={Elsevier}
}

@article{chang2005data,
  title={Data mining of tree-based models to analyze freeway accident frequency},
  author={Chang, Li-Yen and Chen, Wen-Chieh},
  journal={Journal of safety research},
  volume={36},
  number={4},
  pages={365--375},
  year={2005},
  publisher={Elsevier}
}

@article{abellan2013analysis,
  title={Analysis of traffic accident severity using decision rules via decision trees},
  author={Abell{\'a}n, Joaqu{\'\i}n and L{\'o}pez, Griselda and De O{\~n}A, Juan},
  journal={Expert Systems with Applications},
  volume={40},
  number={15},
  pages={6047--6054},
  year={2013},
  publisher={Elsevier}
}

@article{caliendo2007crash,
  title={A crash-prediction model for multilane roads},
  author={Caliendo, Ciro and Guida, Maurizio and Parisi, Alessandra},
  journal={Accident Analysis \& Prevention},
  volume={39},
  number={4},
  pages={657--670},
  year={2007},
  publisher={Elsevier}
}

@article{bergel2013explaining,
  title={Explaining the road accident risk: Weather effects},
  author={Bergel-Hayat, Ruth and Debbarh, Mohammed and Antoniou, Constantinos and Yannis, George},
  journal={Accident Analysis \& Prevention},
  volume={60},
  pages={456--465},
  year={2013},
  publisher={Elsevier}
}

@article{eisenberg2004mixed,
  title={The mixed effects of precipitation on traffic crashes},
  author={Eisenberg, Daniel},
  journal={Accident analysis \& prevention},
  volume={36},
  number={4},
  pages={637--647},
  year={2004},
  publisher={Elsevier}
}

@inproceedings{chen2016learning,
  title={Learning deep representation from big and heterogeneous data for traffic accident inference},
  author={Chen, Quanjun and Song, Xuan and Yamada, Harutoshi and Shibasaki, Ryosuke},
  booktitle={Thirtieth AAAI conference on artificial intelligence},
  year={2016}
}



@inproceedings{najjar2017combining,
  title={Combining satellite imagery and open data to map road safety},
  author={Najjar, Alameen and Kaneko, Shun’ichi and Miyanaga, Yoshikazu},
  booktitle={Thirty-First AAAI Conference on Artificial Intelligence},
  year={2017}
}

2021 Here Map, categories \url{https://developer.here.com/documentation/places/dev_guide/topics/categories.html}
@misc{category,
  title = {{2021 Here Map, categories}},
  howpublished = {\url{https://developer.here.com/documentation/places/dev_guide/topics/categories.html}},
}


@article{HochreiterSepp1997LSM,
issn = {1530-888X},
abstract = {Learning to store information over extended time intervals by recurrent backpropagation takes a very long time, mostly because of insufficient, decaying error backflow. We briefly review Hochreiter's (1991) analysis of this problem, then address it by introducing a novel, efficient, gradient based method called long short-term memory (LSTM). Truncating the gradient where this does not do harm, LSTM can learn to bridge minimal time lags in excess of 1000 discrete-time steps by enforcing constant error flow through constant error carousels within special units. Multiplicative gate units learn to open and close access to the constant error flow. LSTM is local in space and time; its computational complexity per time step and weight is
O
. 1. Our experiments with artificial data involve local, distributed, real-valued, and noisy pattern representations. In comparisons with real-time recurrent learning, back propagation through time, recurrent cascade correlation, Elman nets, and neural sequence chunking, LSTM leads to many more successful runs, and learns much faster. LSTM also solves complex, artificial long-time-lag tasks that have never been solved by previous recurrent network algorithms.},
journal = {Neural computation},
pages = {1735--1780},
volume = {9},
publisher = {MIT Press},
number = {8},
year = {1997},
title = {Long Short-Term Memory},
copyright = {1997 Massachusetts Institute of Technology},
language = {eng},
address = {Cambridge, MA},
author = {Hochreiter, Sepp and Schmidhuber, Jürgen},
keywords = {Algorithmics. Computability. Computer arithmetics ; Algorithms ; Applied sciences ; Artificial intelligence ; Computer science; control theory; systems ; Connectionism. Neural networks ; Exact sciences and technology ; Learning ; Memory ; Memory, Short-Term ; Models, Neurological ; Models, Psychological ; Nerve Net - physiology ; Neural Networks (Computer) ; Theoretical computing ; Time Factors},
}

@inproceedings{10.5555/2969239.2969329,
author = {Shi, Xingjian and Chen, Zhourong and Wang, Hao and Yeung, Dit-Yan and Wong, Wai-kin and Woo, Wang-chun},
title = {Convolutional LSTM Network: A Machine Learning Approach for Precipitation Nowcasting},
year = {2015},
publisher = {MIT Press},
address = {Cambridge, MA, USA},
abstract = {The goal of precipitation nowcasting is to predict the future rainfall intensity in
a local region over a relatively short period of time. Very few previous studies have
examined this crucial and challenging weather forecasting problem from the machine
learning perspective. In this paper, we formulate precipitation nowcasting as a spatiotemporal
sequence forecasting problem in which both the input and the prediction target are
spatiotemporal sequences. By extending the fully connected LSTM (FC-LSTM) to have
convolutional structures in both the input-to-state and state-to-state transitions,
we propose the convolutional LSTM (ConvLSTM) and use it to build an end-to-end trainable
model for the precipitation nowcasting problem. Experiments show that our ConvLSTM
network captures spatiotemporal correlations better and consistently outperforms FC-LSTM
and the state-of-the-art operational ROVER algorithm for precipitation nowcasting.},
booktitle = {Proceedings of the 28th International Conference on Neural Information Processing Systems - Volume 1},
pages = {802–810},
numpages = {9},
location = {Montreal, Canada},
series = {NIPS'15}
}

@inproceedings{10.5555/3001460.3001507,
author = {Ester, Martin and Kriegel, Hans-Peter and Sander, J\"{o}rg and Xu, Xiaowei},
title = {A Density-Based Algorithm for Discovering Clusters in Large Spatial Databases with Noise},
year = {1996},
publisher = {AAAI Press},
abstract = {Clustering algorithms are attractive for the task of class identification in spatial
databases. However, the application to large spatial databases rises the following
requirements for clustering algorithms: minimal requirements of domain knowledge to
determine the input parameters, discovery of clusters with arbitrary shape and good
efficiency on large databases. The well-known clustering algorithms offer no solution
to the combination of these requirements. In this paper, we present the new clustering
algorithm DBSCAN relying on a density-based notion of clusters which is designed to
discover clusters of arbitrary shape. DBSCAN requires only one input parameter and
supports the user in determining an appropriate value for it. We performed an experimental
evaluation of the effectiveness and efficiency of DBSCAN using synthetic data and
real data of the SEQUOIA 2000 benchmark. The results of our experiments demonstrate
that (1) DBSCAN is significantly more effective in discovering clusters of arbitrary
shape than the well-known algorithm CLAR-ANS, and that (2) DBSCAN outperforms CLARANS
by a factor of more than 100 in terms of efficiency.},
booktitle = {Proceedings of the Second International Conference on Knowledge Discovery and Data Mining},
pages = {226–231},
numpages = {6},
keywords = {clustering algorithms, arbitrary shape of clusters, handling nlj4-275oise, efficiency on large spatial databases},
location = {Portland, Oregon},
series = {KDD'96}
}

@INPROCEEDINGS{8970742,
  author={Zhang, Yingxue and Li, Yanhua and Zhou, Xun and Kong, Xiangnan and Luo, Jun},
  booktitle={2019 IEEE International Conference on Data Mining (ICDM)}, 
  title={TrafficGAN: Off-Deployment Traffic Estimation with Traffic Generative Adversarial Networks}, 
  year={2019},
  volume={},
  number={},
  pages={1474-1479},
  doi={10.1109/ICDM.2019.00193}}
  
@book{CressieNoel1993SfSD,
publisher = {John Wiley & Sons, Incorporated},
isbn = {9780471002550},
year = {1993},
title = {Statistics for Spatial Data},
language = {eng},
address = {New York},
author = {Cressie, Noel},
keywords = {Mathematics ; Spatial analysis ; Spatial analysis (Statistics) ; Statistics},
}

@article{lin2015novel,
  title={A novel variable selection method based on frequent pattern tree for real-time traffic accident risk prediction},
  author={Lin, Lei and Wang, Qian and Sadek, Adel W},
  journal={Transportation Research Part C: Emerging Technologies},
  volume={55},
  pages={444--459},
  year={2015},
  publisher={Elsevier}
}
